Evidentiality-guided Generation for Knowledge-Intensive NLP Tasks

Retrieval-augmented generation models have shown state-of-the-art performance across many knowledge-intensive NLP tasks such as open question answering and fact verification. These models are trained to generate the final output given the retrieved passages, which can be irrelevant to the original query, leading to learning spurious cues or answer memorization. This work introduces a method to incorporate the evidentiality of passages -- whether a passage contains correct evidence to support the output -- into training the generator. We introduce a multi-task learning framework to jointly generate the final output and predict the evidentiality of each passage, leveraging a new task-agnostic method to obtain silver evidentiality labels for supervision. Our experiments on five datasets across three knowledge-intensive tasks show that our new evidentiality-guided generator significantly outperforms its direct counterpart with the same-size model and advances the state of the art on FaVIQ-Ambig. We attribute these improvements to both the auxiliary multi-task learning and silver evidentiality mining techniques.

==> sections/background.tex <==
\section{Background}

\paragraph{Set up of retrieval-augmented generation.}
A retrieval-augmented generation framework consists of two components, a retriever model  $\mathcal{R}$ and a generator model $\mathcal{G}$. 
It first trains $\mathcal{R}$ and then retrieve a set of passages $\mathbf{P}$ for each training query $x$: $\mathbf{P} = \mathcal{R}(x)$. 
$\mathcal{G}$ is then trained to generate final output $y$ given $x$ and $\mathbf{P}$ in an weakly-supervised manner: $ y = \mathcal{G}(x, \mathbf{P})$ . 
The framework can be trained for any task given the input-output pair $(x,y)$, and it has shown competitive across many different knowledge-intensive NLP tasks such as open QA~\cite{guu2020realm,lewis2020retrieval,izacard2020distilling,izacard2020leveraging}, fact verification~\cite{lewis2020retrieval}, slot filling~\cite{glass2021zero}, or dialogue~\cite{paranjape2021hindsight}. 
In this work, we base our model on the Fusion-in-Decoder model~\cite[FiD][]{izacard2020leveraging}, a state-of-the-art retrieval-augmented QA model that independently encodes and scale up to many passages (e.g., 100 passages) and generate answers conditioned on those many retrieved passages, demonstrating its competitiveness on open QA. 


\paragraph{Analyses on a model's behavior.}
We conducted a detailed analysis on  FiD. 
We first analyzed FiD's attention scores over $\mathbf{P}$, and found on average, FiD only gives its highest attention scores to the passages ranked at on average 4.8, and in 50\% of the cases gives the highest attention scores to the top one retrieved passages. 
We also found only 5\% of the cases, it gives the highest attention scores to the passages ranked lower than 25. 

We then manually analyze the 50 error cases where sufficient evidence is presented in the retrieved context but FiD fails to generate the correct answer. 
We found that FiD is often fooled by and pays more attention to the higher-ranked false passages with more lexical overlap than the correct evidence passage, resulting in the final generation errors. 
We also found that in error cases, FiD generates arbitrary answers that are not sub-strings of any of the retrieved context from answer memorization five times more frequently than the daftest average, which is consistent with findings of \citet{lewis-etal-2021-question} and \citet{longpre2021entitybased}. 
In those cases, often plausible but hallucinated answers are generated. 
See analysis details and examples in Appendix. 
